Black-Box Optimization for Identifying and Inverting Audio Dynamic Range Control Effects

Dynamic Range Compression (DRC) is a widely used nonlinear audio effect whose parameters are often unknown, making blind estimation and inversion challenging. In this work, we formulate DRC parameter estimation as a black-box optimization problem in a perceptually motivated feature space. Given an observed signal and a reference representation, we estimate the parameters that minimize the distance between feature descriptors of the reconstructed and reference signals. Unlike gradient-based approaches, the proposed method does not require differentiability of the DRC model or the feature extraction pipeline, enabling the use of nonlinear and histogram-based descriptors. Experimental results demonstrate that the proposed method achieves competitive performance in blind parameter estimation and dry signal recovery, outperforming or matching state-of-the-art models in terms of reconstruction quality.

==> DRC.tex <==
\begin{picture}(0,0)%
\includegraphics{figs/DRC.pdf}%
\end{picture}%
%
%  Created by WinFIG version 7.4 
%  METADATA <version>1.0</version> 
%
\setlength{\unitlength}{4460sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(7191,2164)(466,-2888)
%  METADATA <id>1</id> 
\put(481,-1021){\makebox(0,0)[lb]{\smash{{\SetFigFont{14}{16.8}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}$x[n]$}%
}}}}
%  METADATA <id>2</id> 
\put(2011,-1861){\makebox(0,0)[lb]{\smash{{\SetFigFont{14}{16.8}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}Level}%
}}}}
%  METADATA <id>3</id> 
\put(1900,-2070){\makebox(0,0)[lb]{\smash{{\SetFigFont{14}{16.8}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}detector}%
}}}}
%  METADATA <id>8</id> 
\put(3721,-1898){\makebox(0,0)[lb]{\smash{{\SetFigFont{14}{16.8}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}Static}%
}}}}
%  METADATA <id>9</id> 
\put(3728,-2111){\makebox(0,0)[lb]{\smash{{\SetFigFont{14}{16.8}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}curve}%
}}}}
%  METADATA <id>11</id> 
\put(1816,-2806){\makebox(0,0)[lb]{\smash{{\SetFigFont{14}{16.8}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}$\tau_v^{att}$}%
}}}}
%  METADATA <id>13</id> 
\put(2486,-2788){\makebox(0,0)[lb]{\smash{{\SetFigFont{14}{16.8}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}$\tau_v^{rel}$}%
}}}}
%  METADATA <id>14</id> 
\put(2864,-1816){\makebox(0,0)[lb]{\smash{{\SetFigFont{14}{16.8}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}$v[n]$}%
}}}}
%  METADATA <id>20</id> 
\put(5266,-1846){\makebox(0,0)[lb]{\smash{{\SetFigFont{14}{16.8}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}Smoothing}%
}}}}
%  METADATA <id>21</id> 
\put(5540,-2095){\makebox(0,0)[lb]{\smash{{\SetFigFont{14}{16.8}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}filter}%
}}}}
%  METADATA <id>26</id> 
\put(5178,-2680){\makebox(0,0)[lb]{\smash{{\SetFigFont{14}{16.8}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}$\tau_g^{att}$}%
}}}}
%  METADATA <id>27</id> 
\put(6055,-2697){\makebox(0,0)[lb]{\smash{{\SetFigFont{14}{16.8}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}$\tau_v^{rel}$}%
}}}}
%  METADATA <id>28</id> 
\put(4576,-1841){\makebox(0,0)[lb]{\smash{{\SetFigFont{14}{16.8}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}$f[n]$}%
}}}}
%  METADATA <id>33</id> 
\put(3646,-1043){\makebox(0,0)[lb]{\smash{{\SetFigFont{14}{16.8}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}Delay}%
}}}}
%  METADATA <id>45</id> 
\put(6587,-1039){\makebox(0,0)[lb]{\smash{{\SetFigFont{14}{16.8}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}$\times$}%
}}}}
%  METADATA <id>50</id> 
\put(7642,-944){\makebox(0,0)[lb]{\smash{{\SetFigFont{14}{16.8}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}$y[n]$}%
}}}}
%  METADATA <id>51</id> 
\put(6774,-1870){\makebox(0,0)[lb]{\smash{{\SetFigFont{14}{16.8}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}$g[n]$}%
}}}}
\end{picture}%

